Designing Adaptive Developer-Chatbot Interactions: Context Integration, Experimental Studies, and Levels of Automation

The growing demand for software developers and the increasing development complexity have emphasized the need for support in software engineering projects. This is especially relevant in light of advancements in artificial intelligence, such as conversational systems. A significant contributor to the complexity of software development is the multitude of tools and methods used, creating various contexts in which software developers must operate. Moreover, there has been limited investigation into the interaction between context-based chatbots and software developers through experimental user studies. Assisting software developers in their work becomes essential. In particular, understanding the context surrounding software development and integrating this context into chatbots can lead to novel insight into what software developers expect concerning these human-chatbot interactions and their levels of automation. In my research, I study the design of context-based adaptive interactions between software developers and chatbots to foster solutions and knowledge to support software developers at work.

==> aspectsIdentification.tex <==

\textbf{------- From now on, this information will be used for analysis but will not be in the paper}
Sheridan and Verplank \cite{sheridan1978human} identified, in 1978, six functions that either a human operator or a computer could maintain during teleoperation control (gets, selects, starts, requests, approves and tells). Based on these functions, humans and computers should cooperate and change roles under different LOAs. As a result, they introduce 10 LOA levels, varying from fully manual to fully computer automated. As of the elements mentioned that impact the decisions, we were able to identify the following: 
\begin{itemize}
\item Communication
\item Task complexity 
\item Handling qualities: responsiveness, interface transparency, naturalness, dexterity, flexibility, gracefulness in failure 
\item Operator mental workload 
\item Feedback
\end{itemize}

In 1987, Endsley \cite{endsley1987application} presented a taxonomy of 4 LOA for a cockpit to supplement human decision-making (the pilot) for automated systems control. She identified 4 functions (suggest, concur, veto and act) during which the human operator or the machine could be in charge. Following Endsley's approach, Ntuen and Park \cite{ntuen1996human} added a fully manual level. Their approach consists then of 5 levels, 4 of which are identical to Endsley's. As of the elements mentioned that impact the decisions of if the human or machine is in charge, we were able to identify the following: 
\begin{itemize}
\item Human workload
\item Situational awareness (SA)
\item Task Frequency
\item Performance 
\item Human acceptance of the system  %TODO checar synonym / discutir com Paulo
\end{itemize}

In the specific case of following a system breakdown or failure, Endsley and Kiris \cite{EndsleyKiris1995} suggested that other factors suggest that implementing automation while maintaining a high level of control for the human operator provides definite benefits in minimizing the out-of-the-loop performance problem, as compared with full automation. Therefore, considering: 
\begin{itemize}
\item Situation awareness and
\item Decision time
\end{itemize}
after a system failure could potentially impact which level of automation to pursue. Later, another study \cite{endsley1999level} provides an indication of the relevant task aspects that may influence the success or failure of automation efforts that seek to create an effective human/machine system and provide a smooth transition during automation failures. This study considered the following elements:
\begin{itemize}
\item Task performance during normal operation
\item Task performance in failure
\item Operator situation awareness
\item Operator perceived workload
\end{itemize}

Riley \cite{riley1989general} published, in 1989, an approach that introduced the idea of the system's intelligence. They presented as a 2-D matrix, where the rows correspond to the LOA (how much autonomy it has) and the columns correspond to Levels of Intelligence (how intelligent the automation is). The combination of these levels is called the "automation state". They proposed 12 automation levels, respecting the boundaries of fully autonomous and fully manual levels. They propose a model with elements that impact the behaviour of the machine or human decisions on automation, namely:
\begin{itemize}
\item Operator workload levels
\item Risk levels
\item Task complexity
\item Operator skill levels
\item Trust and perceived reliability
\end{itemize}

Miligram et al. \cite{Milgram1995} propose 5 levels of automation for remote control operations. With a yet not seen taxonomy for describing the levels, the authors consider the role that humans could play when controlling machines. They propose a model with elements that impact the behaviour of the machine or human decisions on automation, namely:
\begin{itemize}
\item Environment knowledge (abstracting to SA) 
\item Role/Authority of the human operator
\end{itemize}

In their work, Draper \cite{draper1995teleoperators} suggests 9 levels of automation for advanced manufacturing, and considers the following elements that impact the behaviour of the machine or human decision: 
\begin{itemize}
\item Environment variability
\item Environment accessibility
\item Environment structure
\end{itemize}

Similarly to research on the level of automation after a system failure \cite{EndsleyKiris1995,endsley1999level}, Lorenz et al. \cite{lorenz2001effects} studied the reasoning behind automation decisions during/after a system failure or fault and recovery. The elements considered to support the decisions were: 
\begin{itemize}
\item Perceived tension (calm vs. tense)
\item Fatigue (alert vs. tired)
\item Subjective workload
\item Trust and self-confidence
\end{itemize}



Demir et al. \cite{demir2017team} investigate how team interaction (i.e. verbal behaviors) affects heterogeneous teams composed of human and autonomous systems. The authors compared a team composed of only humans against a heterogeneous team, assessing different team verbal behaviors that are usually associated with team coordination, ranging from the ability of just repeating a request to making suggestions and planning ahead. The authors illustrated their approach with three scenarios in the context of unmanned aerial vehicles (UAV), varying the synthetic condition of the pilot (whether the pilot is synthetic or human), who is responsible for the main task in this application scenario. Accordingly, the human-autonomy teams had lower levels of team verbal behavior than all-human teams. 

\begin{itemize}
    \item Interaction ways: verbal behaviors that are associated to team coordination. Pushing and pulling information (information push is the behavior of anticipating the information that another member of the team needs). Push (general status - informing other team members about current status; suggestions - make suggestions to the other team members; planning ahead - anticipating next steps and creating rules); Pull (repeated requests - Requesting the same information or action from other team member(s); Inquiry about status of others - 'Inquiring about current status of others, and expressing concerns ')
    \item Application scenario: Unmanned Aerial Vehicles (UAV)
    \item Task Evaluation Score: team performance measures (mission performance score), team process measure (team coordination, process rating, situation awareness), and other measures ("taskwork and teamwork knowledge, NASA-TLX workload measure \cite{hart2006nasa} and post-experiment questionnaire")
    \item Behavior: verbal communication, cooperation through pushing and pulling information
\end{itemize}

Clough \cite{clough2002metrics} presents some metrics to evaluate autonomy in the context of Unmanned Aerial Vehicles. 
% olhar tabela 3 desse artigo pq ele mostra diferentes tipos de perception, analysis e cooperation. https://apps.dtic.mil/sti/pdfs/ADA515926.pdf
\begin{itemize}
    \item Interaction ways: 
    \item Types of Supervision: rejection of plan, ask for abort/recall, fully independent, Health Status monitored by external supervision, External control via low level commands
    \item Types of Cooperation: hierarchical cooperation with other autonomous systems
    \item Application scenario: Unmanned Aerial Vehicles (UAV)
    \item Task Evaluation Score: 
    \item Behavior: Task planning (reactive behavior); perception/situational awareness (based on the number of sensors); analysis/decision making (e.g. full decision making on-board; evaluation and replan); communication/cooperation; act; self-health-diagnosis  - comentario meu: cada um desses behaviors representam grupo de behaviors, pq se ele tiver o behavior de perception, isso varia de acordo com o numero de sensores; decision varia de acordo com os modelos de decisao/algoritmos q ele pode ter
    task planning (e.g., interprete goals into actions, multi-agent collaboration), situational awareness (e.g., single sensor) \cite{clough2002metrics}. ...There are 3 stages of situational awareness: information gathering, understanding information, and anticipation.
    \item Autonomous System Attributes: mobility control (e.g., operator assisted, do one command, integrate multiple actions), fault/event adaptive, robust response to anticipated event, limited response to real time faults/events, pre-loaded alternative plans, remotely controled, execute preplanned mission; assistance (i.e. requires little guidance, no supervisory assistance, minimal supervisory assistance); event-driven
    \item Limitations: limited response to real time faults/events
\end{itemize}


Fereidunian et al. \cite{fereidunian2007challenges} 

\begin{itemize}
    \item Interaction ways: 
    \item Application scenario: Electric power utility management 
    \item Task Evaluation Score: 
    \item Behavior: 
    \item types of control: the autonomous system ignores the human; the system decides whether to inform/contact the human; the system informs the human about the action only if the human asks; for every action, the system informs the human; the system gives to the human a restricted time to veto before executing the task; the system needs the human approval before executing the task; the system provides the best solution for the task, but the human executes it; the system just identifies the fault location, so the humam can solve it by themselves; manual operation 
    \item Tasks: information processing, decision support, decision making, and action implementation 
\end{itemize}


Proud et al. \cite{proud2003methods}

\begin{itemize}
    \item trust
    \item cost/benefit of the implementation
\end{itemize}

\textbf{Vagia et al. : forward analysis
}

Nylin et al. \cite{Nylin2022261}
\begin{itemize}
    \item manage system breakdown (recovery ability)
    \item human cognitive ability
    \item time to control x time to change process
\end{itemize}

Calhoun \cite{Calhoun2022269}
\begin{itemize}
    \item human / task workload
    \item fatigue
    \item anxiety
    \item confidence
    \item skill
    \item sa
    \item human engagement
    \item system timely automated changes 
    \item recovery after fail 
    \item context (domain characteristics)
\end{itemize}


Villani et al. \cite{Villani20211969}
\begin{itemize}
    \item tasks
    \item environment
    \item hardware
    \item user capability
    \item user comfort to do the task
    \item time-lapse
    \item performance degradation
    \item age
    \item disability
    \item experience
    \item anxiety, fear, boredom, fatigue, exhaustion
    \item worker's mental and phisical fatigue
    \item progress in process
    \item skills, cognitive load, visual attention
\end{itemize}


Novakazi et al. \cite{Novakazi2021116}
\begin{itemize}
    \item the context
    \item the vehicle
    \item the driver
    \item Specific:
    \item Driver Tasks (The Driver
Tasks aspect was divided into two sub-aspects,
namely Interaction with Displays and Controls
and Operation of Vehicle)
    \item Vehicle Operations
    \item Abilities and Limitations of the Systems
    \item the Attentional Demand Required from the Driver
    \item Control of the Vehicle
    \item Driving Context (the Driving
Context was divided into Traffic Conditions and
Road Types.)
\end{itemize}


Keiser et al. \cite{Keiser2021413}
\begin{itemize}
    \item paper is not in english
\end{itemize}

Simmler et al. \cite{Simmler2021239} 
\begin{itemize}
    \item task
    \item environment
    \item system transparency
    \item indetermination
    \item adaptability
    \item openness 
\end{itemize}

Müller et al. \cite{Muller20213}
\begin{itemize}
    \item systematic process (ability to execute modeled process)
    \item adaptability
    \item self-governance
    \item self-containedness
    \item LOOK AT FIGURE 2 IN THIS PAPER BEFORE GOING TO THE NEXT STEP. 
\end{itemize}

Ramos et al. \cite{Ramos2020629}
\begin{itemize}
    \item safety
    \item task
\end{itemize}

AitMalek et al. \cite{AitMalek2020408}
\begin{itemize}
    \item operating cost of equipment
    \item labor cost
\end{itemize}

Ahmadi-Karvigh et al. \cite{Ahmadi-Karvigh2017163}
\begin{itemize}
    \item task
    \item context
    \item workload
\end{itemize}


\textbf{Simmler et al. \cite{Simmler2021239} - Backwards analysis: }
%% parei aqui
Beer et al. \cite{beer2014toward}
\begin{itemize}
    \item situation awareness, workload, acceptance, trust and acceptance, robot’s intelligence and learning capabilities, robot reliability, transparency, social skills
\end{itemize}
Castelfranchi et al. \cite{castelfranchi2003founding}
\begin{itemize}
    \item Agent architecture (and by skills, knowledge, cognitive capabilities, etc.); external resources are provided (or limited) by accessibility, competition, pro-social relations, and norms.
\end{itemize}
Flemisch et al. \cite{flemisch2012towards}
\begin{itemize}
    \item ability, authority, control and responsibility,
\end{itemize}
Kaber et al. \cite{kaber2018issues}
\begin{itemize}
    \item  human performance, workload, and situation awareness
\end{itemize}
Parasuraman et al. \cite{parasuraman2000model}
\begin{itemize}
    \item  information acquisition, information analysis, decision selection, and action implementation.
\end{itemize}

\textbf{Simmler et al. \cite{Simmler2021239} - Forward analysis: }
Khuat et al. \cite{khuat2022roles}
\begin{itemize}
    \item accessibility,
transparency, fairness, reliability, systemn(workload, engagement, complexity), system design (automation robustness, automation reliability), environment (competing tasks, demands), cognitive construct (situation awareness, mental model, attention allocation, automation trust)
\end{itemize}

==> stateoftheart.tex <==
\section{State of the Art} \label{background}


\subsection{Levels of Automation} 

Automation has been implemented and desired in a variety of systems, aiming at improving the performance of the tasks executed and overcoming heavy human workloads \cite{Endsley1997}. Retaining the human-in-the-loop with well-designed tasks that humans can perform well is also desired, as an effort to improve system functioning \cite{endsley1999level}. 


Reescrever - "Autonomy is a system independent of human control (i.e., it makes its own decisions about its actions during the task), whereas automation is a system that will do exactly what it is programmed without independent action" \cite{demir2017team}

\textbf{Discuss autonomy x automation}

"The human-centered automation (HCA) design approach seeks the optimum collaboration between the human and the computer, instead of the older attitude of substituting human by computer and leaving the un-automatable tasks for the human operator "
"The human-machine job allocation has been considered as a classic problem, since the early days of very basic automation;"

\subsection{Conversational Agents \& Autonomous Systems }

Autonomous Systems may have/operate with levels of autonomy... 

\subsection{Variability Aware Approaches} 
%- mention here why feature models make sense in this work; highly configurable systems; avoid rebuilding a new system; highly dynamic systems are not desired as well

Variability is the ability of a software system to be configured for different contexts and scenarios \cite{galster2013variability}. The first step to achieving variability in a system is understanding and representing variability in its application domain. Our approach incorporates feature oriented domain analysis (FODA) \cite{pohl2005software} to represent software variability. According to the FODA notation, we can classify features as mandatory, optional, and alternative.

%\subsubsection{Feature Model}



\subsection{Issues in Human-Autonomy \&& Autonomous Systems}

According to Demir et al. \cite{demir2017team}, the Human-Autonomy Teaming (HAT) has some costs and benefits. Despite autonomous systems increase the work productivity, their agents' lack of human-like behavior can place high cognitive demands on human teammates.

Another problem is the limited language capability of autonomous systems, such as difficulty in understanding ambiguous and cryptic expressions. This situation can cause the system to need more time to understand the situation, or even cause the system to fail. %misunderstanding

A study performed by Endsley and Kiris \cite{EndsleyKiris1995} indicates that humans were slower to perform a high-cognitive task manually following the breakdown of the automated system than if they had been performing manually all along. 


% file:///Users/gmelo/Nextcloud/Downloads-cloud/baez2020-chatbot-integration-patterns.pdf
% Chatbot integration in few patterns
% Marcos Baez
% Université Claude Bernard Lyon, Lyon, France


% https://link.springer.com/article/10.1007/s00607-021-01016-7

% https://towardsdatascience.com/how-to-build-your-own-chatbot-using-deep-learning-bb41f970e281

% Intents: https://arxiv.org/abs/2201.02735

% SLR: file:///Users/gmelo/Nextcloud/Downloads-cloud/information-13-00041-v2.pdf

% cool drawing on chatbot architecture: 
% https://www.youtube.com/watch?v=X3s0NC7fSoE
% https://www.youtube.com/watch?v=XFARym8bleE

% ---- LOA: 
% https://www.proquest.com/openview/bd68655e0a2bbeda8d7e1bf406b42447/1?pq-origsite=gscholar&cbl=47901

% https://ieeexplore.ieee.org/document/8304784

% \subsection{Chatbots for Software Engineering}
% Some researchers have proposed the use of chatbots to automate different software engineering (SE) tasks or to assist software engineers with their tasks. These investigations include approaches to: i) project management \cite{hefny2021proactive}; mining software repositories \cite{assavakamhaenghan2021interactive}; 
% Abdellatif et al. \cite{abdellatif2021comparison} investigate different Natural Language Understanding (NLU) component to be used in chatbots deployed at 
% three aspects (intents classification, confidence scores, and entity extraction)


==> table.tex <==
% Please add the following required packages to your document preamble:

\begin{table*}[ht]
\footnotesize	
\centering
\caption{Preliminary LOA Factors and Authors which cited each factor.}
\label{tab:aspectstable}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Factors} &  &  & \textbf{Authors} \\ \midrule
\textbf{Quality} &  &  &  \\
 & Trust &  & \cite{proud2003methods}\cite{beer2014toward} \\
 & Reliability &  & \cite{sheridan1978human}\cite{khuat2022roles} \\
 & Fairness &  & \cite{khuat2022roles} \\ \midrule
\textbf{Task} &  &  &  \\
 & Result &  & \cite{Simmler2021239}\cite{Ramos2020629}\cite{Ahmadi-Karvigh2017163} \\
 & Quality &  & \cite{Simmler2021239}\cite{Ramos2020629}\cite{Ahmadi-Karvigh2017163} \\
 &  & Performance & \cite{endsley1987application}\cite{endsley1999level} \\ \midrule
\textbf{Agent} &  &  &  \\
 & Cost &  & \cite{AitMalek2020408}\cite{proud2003methods} \\
 & Communication (verbal) &  & \cite{sheridan1978human}\cite{demir2017team} \cite{clough2002metrics} \\ \midrule
\textbf{Human} &  &  &  \\
 & Age &  & \cite{Villani20211969} \\
 & Control timing &  & \cite{Nylin2022261} \\
 & Cognitive Ability &  & \cite{Nylin2022261}\cite{Villani20211969}\cite{castelfranchi2003founding} \\ \midrule
\textbf{Environment} &  &  & \cite{Simmler2021239} \\
 & Variability &  & \cite{draper1995teleoperators}\cite{Villani20211969}\cite{Simmler2021239} \\
 &  & Unchanging/Highly Dynamic & \cite{draper1995teleoperators} \\
 & Competing tasks &  & \cite{khuat2022roles} \\
 & Demands &  & \cite{khuat2022roles} \\ \bottomrule
\end{tabular}%
}
\end{table*}

